Polarized Raman spectroscopy study of metallic $(Sr_{1-x}La_{x})_{3}Ir_{2}O_{7}$: a consistent picture of disorder-interrupted unidirectional charge order

We have used rotational anisotropic polarized Raman spectroscopy to study the symmetries, the temperature and the doping dependence of the charge ordered state in metallic $(Sr_{1-x}La_{x})_{3}Ir_{2}O_{7}$. Although the Raman probe size is greater than the charge ordering length, we establish that the charge ordering breaks the fourfold rotational symmetry of the underlying tetragonal crystal lattice into twofold, as well as the translational symmetry, and forms short-range domains with $90^{\circ}$ rotated charge order wave vectors, as soon as the charge order sets in below $T_{CO} = \sim$ 200K and across the doping-induced insulator metal transition. We observe that this charge order mode frequency remains nearly constant over a wide temperature range and up to the highest doping level. These above features are highly reminiscent of the ubiquitous unidirectional charge order in underdoped high-$T_C$ copper-oxide-based superconductors (cuprates). We further resolve that the charge order damping rate diverges when approaching $T_{CO}$ from below and increases significantly as increasing the La doping level, which resembles the behaviors for a disorder-interrupted ordered phase and has not been observed for the charge order in cuprates.

==> arxiv file/author_list.tex <==
% Author list

\author{Wencan Jin}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, Michigan 48109, USA}

\author{Siwen Li}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, Michigan 48109, USA}

\author{Jianpeng Liu}
\affiliation{Kavli Institute of Theoretical Physics, University of California, Santa Barbara, California 93106, USA}

\author{Qiang Han}
\affiliation{Department of Physics and Astronomy, Rutgers University, Piscataway, New Jersey 08854, USA}

\author{Zach Porter}
\affiliation{Materials Department, University of California, Santa Barbara, California 93106, USA}

\author{Christi Peterson}
\affiliation{Materials Department, University of California, Santa Barbara, California 93106, USA}

\author{Julian Schmehr}
\affiliation{Materials Department, University of California, Santa Barbara, California 93106, USA}

\author{Ibrahim Boulares}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, Michigan 48109, USA}

\author{Kai Sun}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, Michigan 48109, USA}

\author{Roberto Merlin}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, Michigan 48109, USA}

\author{Stephen D. Wilson}
\affiliation{Materials Department, University of California, Santa Barbara, California 93106, USA}

\author{Liuyan Zhao} 
\email{lyzhao@umich.edu}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, Michigan 48109, USA}
